Towards Understanding the Bugs in Solidity Compiler

Solidity compiler plays a key role in enabling the development of smart contract applications on Ethereum by governing the syntax of a domain-specific language called Solidity and performing compilation and optimization of Solidity code. The correctness of Solidity compiler is critical in fostering transparency, efficiency, and trust in industries reliant on smart contracts. However, like other software systems, Solidity compiler is prone to bugs, which may produce incorrect bytecodes on blockchain platforms, resulting in severe security concerns. As a domain-specific compiler for smart contracts, Solidity compiler differs from other compilers in many perspectives, posing unique challenges to detect its bugs. To understand the bugs in Solidity compiler and benefit future research, in this paper, we present the first systematic study on 533 Solidity compiler bugs. We carefully examined their characteristics (including symptoms, root causes, and distribution), and their triggering test cases. Our study leads to seven bug-revealing takeaways for Solidity compiler. Moreover, to study the limitations of Solidity compiler fuzzers and bring our findings into practical scenarios, we evaluate three Solidity compiler fuzzers on our constructed benchmark. The results show that these fuzzers are inefficient in detecting Solidity compiler bugs. The inefficiency arises from their failure to consider the interesting bug-inducing features, bug-related compilation flags, and test oracles

==> CODE/OptimizationError.tex <==
{
  foo(2)
  function foo(x)
  {
    mstore(0, shl(1,shl(not(0),x)))
  }
}

==> CODE/PEM.tex <==
Uncaught exception:
Dynamic exception type: std::bad_cast
std::exception::what: std::bad_cast

==> CODE/PEM2.tex <==
Error: Expected an inline tuple, not an expression of a tuple type. --> test1.sol:10:32:
10  abi.encodeCall(this.f, g0());  // bad_cast

==> CODE/RVP.tex <==
TypeError: Construction control flow ends without initializing all immutable state variables.
  --> tests/remix_tests_test.sol:10:9:
   |
10 |         return;
Note: Not initialized: 
  --> tests/remix_tests_test.sol:15:5:
   |
15 |     uint public immutable baked = 123;

==> CODE/codegenerror.tex <==
contract C {
  function C() {
    f();
  }
  function f() internal {
    uint x = 42;
  }
}

==> CODE/exceptionhandlingerror.tex <==
contract C {
  struct S {
    function() a;
  }
  function f(S[2] calldata) {}
}

==> CODE/fverror.tex <==
contract C {
	uint v;
	bool guard = true;

	function dec() public returns (uint) {
		if (guard) return 0;
		--v;
		return v;
	}

	function f() public returns (uint) {
		guard = false;
		uint ret = this.dec();
		guard = true;
		return ret;
	}
}

==> CODE/incorrect_output.tex <==
contract RevertReasonParserTest {
    function emptyStringRevert() external pure  {
        revert("");
    }

    function test() external view returns(bytes memory, uint256) {
        try this.emptyStringRevert() {
        } catch (bytes memory reason) {
            return (reason, reason.length);
        }
    }
}

==> CODE/memoryissue.tex <==
struct S {
    uint x;
}
contract C {
    S sStorage;
    function f() external {
        S[] memory sMemory;
        sMemory[0] = sStorage;
    }
}

==> CODE/semanticanalysiserror.tex <==
library L {
    function privateFunction(uint) private {}
}
using {L.privateFunction} for unit;

==> CODE/syntaxanalysiserror.tex <==
interface Foo {}
interface Bar {
    event MyEvent(Foo indexed indexed indexed some);
}

==> CODE/typesystemerror.tex <==
contract C {
  function h() public {
    int x;
    ((x**-3));
  }
}

==> figure/fv.tex <==
\begin{figure}[ht]
\centering
    \includegraphics[width=1.0\linewidth]{figure/FV.pdf}
    \caption{The Distribution of Formal Verification Errors over Years} 
    \label{figure:fv}
\end{figure}

==> revision/sec_4_1.tex <==
This section aims to facilitate a deeper understanding of bug characteristics, 
expose underlying bug-revealing characteristics in the collected test cases, and analyze the required test oracles for non-crash symptoms.

==> revision/sec_5_5_old.tex <==
\cref{tab:fuzzing} presents the fuzzing results of 20-day executions on a server with AMD Ryzen Threadripper 3970X 32-Core Processor
, NVIDIA GeForce RTX3090 GPU, and 250G RAM, coordinated
with 64-bit Ubuntu 22.04 OS.
AFL-compiler-fuzzer, through an 8.97\% improvement in the edge coverage of \compiler{} achieved by its seeds, identified one crash in the latest version of the compiler and discovered nine bugs in the benchmark 
. In contrast, solfuzzer, lacking code-structure-aware mutators like AFL-compiler-fuzzer, has a narrower mutation scope, resulting in only a 3.82\% improvement in edge coverage. 
These relatively minor improvements explain the absence of bugs detected by solfuzzer.
Compared with solfuzzer, AFL-compiler-fuzzer carries additional language-agnostic mutation
rules and has a code-splicing helper to enrich the seed pool. 
\wac{I am a bit confused, why the overall edge coverage of solfuzzer is higher than ACF while the increase percentage of ACF is higher?}
% \jj{It seems that only seven bugs are explained. what about the remaining two bugs detected by AFL? The presentation is a bit disordered. We need to separate this long paragraph into some small paragraphs for better illustration.} \haoyang{The remaining 2 bugs are irrelevant for discussion. One is Syntax Analysis Error and the other is Code Generation Error. I cannot extract any information from them since 1) Syntax Analysis Error is not a major root cause, and 2) we don't have a takeaway for revealing codegen error. The only possible takeaway is that codegen error is highly related to incorrect output symptom, which requires a output-aware test oracle. However, this revealed codegen error is a crash.}

Though with these strengths, the bug detection ability of AFL-compiler-fuzzer is inefficient. 
Out of 24 semantic analysis errors and 36 formal verification errors collected in the benchmark, AFL-compiler-fuzzer was able to detect only one semantic analysis error and two formal verification errors.
The relatively high efficiency of AFL-compiler-fuzzer in identifying memory-related errors (four out of 12) stands in stark contrast to its inefficiency in detecting these two significant errors.
The reason for this contrast is that memory-related errors can be easily exposed by utilizing just three memory-related keywords and memory-related operations such as copying across different memory slots (according to takeaway 4). 
On the other hand, detecting the other two errors is more complex as it involves considering factors such as scope, type, and data flow (according to takeaway 2 and 3). AFL-compiler-fuzzer is incapable of extracting such knowledge from seed files, and its mutation strategies are not strong enough to insert such bug-triggering elements,
which contributes to the low efficiency in detecting these errors.
% In addition to armoring these two fuzzers with bug bug-revealing code patterns pointed out by our takeaways, they can evolve by equipping our suggested test oracles \wac{Which oracle? } and utilizing our mentioned bug-related compilation flags to uncover bugs beyond the scope of our benchmark.

==> table/table2.tex <==
\begin{table*}[t]
    \centering
    \small
    \caption{Fuzzing Result
    \victor{I think only display this one is sufficient. }
    }
    \vspace{-2mm}
    \label{tab:fuzzing}
    % \begin{adjustbox}{width=\textwidth,center}
    \ifletter
    \begin{adjustbox}{width=1\textwidth,center}
    \fi
    \begin{tabular}{c|c|c|c|c|c|c|c}
         \toprule
         \textbf{Fuzzer} & \textbf{\#Crash}$_l$  & \textbf{\#Bug}$_b$ & \textbf{\#Hang} & \textbf{Map Density} & \textbf{Line Coverage} & \textbf{Function Coverage} & \textbf{Branch Coverage}
         \\
         % & \textbf{\#Test Cases} \\
         \midrule
         AFL-compiler-fuzzer & 1 & 8 & 0 & 79.93\% ($\Uparrow5.92\%$) & & & \\
         % &21789\\
         solfuzzer & 0 & 0 & 24 & 88.22\% ($\Uparrow3.70\%$) & & &\\
         Fuzzol & 0 & 4 & 10 & 81.00\% ($\Uparrow13.02\%$) & & & \\
         % &10653\\
        \bottomrule
    \end{tabular}
    \ifletter
    \end{adjustbox}
    \fi
    \begin{tablenotes}
    \footnotesize
    \item \textbf{\#Crash}$_l$: the number of revealed crashes in the latest version of \compiler{}
    \item \textbf{\#Bugs}$_b$: the number of detected bugs inside the benchmark
    \item \textbf{\#Hang}: the number of triggered hangs in the latest version of \compiler{}
    % \item \textbf{Coverage}: from left to right, line coverage, function coverage, branch coverage
    % \item \textbf{\#Mutants}$_b$: the number of generated mutants by fuzzers
    % \item \textbf{\#Test Cases}: the number of generated test cases
    \end{tablenotes}
    % \ifletter
    % \end{adjustbox}
    % \fi
    % \vspace{-3mm}

\end{table*}

==> table/table2_old.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{Fuzzing Result}
    \vspace{-2mm}
    \label{tab:fuzzing_old}
    % \begin{adjustbox}{width=0.49\textwidth,center}
    \begin{tabular}{c|c|c|c|c}
         \toprule
         \textbf{Fuzzer} & \textbf{\#Crash}$_l$  & \textbf{\#Bug}$_b$ & \textbf{Edge Coverage} & \textbf{\#Mutants}
         \\
         % & \textbf{\#Test Cases} \\
         \midrule
         ACF & 1 & 9 & 85.62\% ($\Uparrow8.97\%$) & 15669 \\
         % &21789\\
         solfuzzer & 0 & 0 & 92.52\% ($\Uparrow3.82\%$) & 10653 \\
         % &10653\\
        \bottomrule
    \end{tabular}
        \begin{tablenotes}
    \footnotesize
    \item \textbf{ACF} is short for AFL-compiler-fuzzer
    \item \textbf{\#Crash}$_l$: the number of revealed crashes in the latest version of \compiler{}
    \item \textbf{\#Bugs}$_b$: the number of detected bugs inside the benchmark
    \item \textbf{\#Mutants}$_b$: the number of generated mutants by two fuzzers
    % \item \textbf{\#Test Cases}: the number of generated test cases
    \end{tablenotes}
    % \end{adjustbox}
    % \vspace{-3mm}
\end{table}
